Prutor: A System for Tutoring CS1 and Collecting Student Programs for Analysis

An introductory programming course (CS1) is an integral part of any undergraduate curriculum. Due to large number and diverse programming background of students, providing timely and personalised feedback to individual students is a challenging task for any CS1 instructor. The help provided by teaching assistants (typically senior students) is not sufficient as it suffers from unintentional bias and, most of the time, not quick enough. In this paper, we present Prutor, a tutoring system platform to conduct introductory programming courses. Prutor is a cloud-based web application that provides instant and useful feedback to students while solving programming problems. Prutor stores, at regular intervals, the snapshots of students' attempts to solve programming problems. These intermediate versions of the student programs provide the instructors (and data analysts) a view of the students' approach to solving programming problems. Since Prutor is accessible through any standard web browser, students do not need to worry about dependencies external to the programming course, viz. Operating Systems, Editors, Compilers, Compiler Options, etc.. This enables the students to focus on solving only the programming problems. Apart from the code snapshots at regular intervals, Prutor also collects other valuable data such as the time taken by the students to solve the problems, the number of compile and execution events, and the errors made. We have used this data in developing intelligent tools for giving feedback to students, some of which are described briefly in this paper. This system thus serves as a platform for tutoring as well as data collection for researchers.

==> concepts.tex <==
\begin{CCSXML}
    <ccs2012>
    <concept>
    <concept_id>10003120.10003121.10003129</concept_id>
    <concept_desc>Human-centered computing~Interactive systems and tools</concept_desc>
    <concept_significance>500</concept_significance>
    </concept>
    <concept>
    <concept_id>10003120</concept_id>
    <concept_desc>Human-centered computing</concept_desc>
    <concept_significance>300</concept_significance>
    </concept>
    <concept>
    <concept_id>10003120.10003121</concept_id>
    <concept_desc>Human-centered computing~Human computer interaction (HCI)</concept_desc>
    <concept_significance>300</concept_significance>
    </concept>
    <concept>
    <concept_id>10011007.10011074.10011075</concept_id>
    <concept_desc>Software and its engineering~Designing software</concept_desc>
    <concept_significance>500</concept_significance>
    </concept>
    <concept>
    <concept_id>10011007</concept_id>
    <concept_desc>Software and its engineering</concept_desc>
    <concept_significance>300</concept_significance>
    </concept>
    </ccs2012>
\end{CCSXML}

\ccsdesc[500]{Human-centered computing~Interactive systems and tools}
\ccsdesc[300]{Human-centered computing}
\ccsdesc[300]{Human-centered computing~Human computer interaction (HCI)}
\ccsdesc[500]{Software and its engineering~Designing software}
\ccsdesc[300]{Software and its engineering}

\printccsdesc

==> conceptualView.tex <==
CONCEPTUAL FRAMEWORK
DOMAIN LEXICON

Engine: The component of the system which is responsible for tasks such as compilation, execution, evaluation and feedback generation.

Virtual File: An identifier for a student program, created on the system, which appears as a file to the student. Actual files are not created on the disk.

Virtual Folder: An identifier for a collection of programs, created on the system, which appears as a folder to the student. Actual folders are not created on the disk.

Workspace: A collection of virtual files and folders, used by a student for programming purposes.

ScratchPad: A web based IDE interface, wherein a student can create virtual files and folders as a part of her workspace. Students can arbitrary write programs in such files using a provided editor window, in the programming language assigned for the course. These programs can be compiled and their results can be viewed in the form of annotations in the gutter area of the editor window. Compiler messages can be viewed in a virtual console located within the same user interface. Further, the student may execute her compiled program on arbitrary test cases and view the results in an output window, within the same user interface. Execution results such as runtime errors or time limit exceeded errors can also be viewed. 

CodeBook: A portal where students can view submitted solutions to programming assignments along with the corresponding problem statements for course events that were held previously. Grading information for the submitted assignments can also be viewed in the same interface. The portal also contains solutions to practice problems attempted by the student, along with the corresponding problem statements.

Course Event: Any event which is conducted during the course offering, and includes programming assignments to be solved by students. Such events are expected to have a set of programming problems assigned to each student who is enrolled for the course. The events may span multiple days or have multiple schedules. Lab assignments, examinations and quizzes are examples.

Schedule: A time period which corresponds to a course event, during which, members of that schedule may solve the programming problems assigned to them. All programming problems assigned to a particular student for a course event are only accessible to her during the time span of the schedule. 

Practice Problems: A set of problems, which are not associated with any course event. They are accessible at all times, and can be solved by the student at all times. They are intended to provide practice to the students in solving programming problems.

PracticeArena: A portal where a student can access a collection of programming problems for practice. Students may view these problems and navigate to the editor interface, using which they can solve the problem.

Admin: A teaching assistant, tutor or an instructor of the course.

Teaching Assistant: A student who helps the instructor of the course in carrying out activities such as grading, invigilation and helping students solve programming problems.

Tutor: A student or a professor who has the responsibilities of setting questions for various course events and deciding the policies of the course events.

Instructor: A professor who conducts the course. He is responsible for deciding the course structure and grading policies for the course.

GradeCard: A table containing scores awarded by teaching assistants, tutors and instructors for the programming problems that were solved by the student for various course events. These scores are grouped by the course events attended by the student.

Pager: A publish-subscribe based messaging system wherein a student can create a message thread when she requires help in solving programming problems or in addressing technical difficulties, while solving the problems. Instructors, tutors and teaching assistants are able to view these messages and respond to them in real time. Only students can start a message thread, while others can only respond to them.

DataViz: A portal where data collected using the system can be tabulated in arbitrary formats or visualizations may be created from the data.

ControlPanel: A portal from where administrators can tune the settings of the Engine. Settings include time delays in compilation and execution along with execution quotas, compiler flags and tool active state.

CodeViewer: An user interface where the code history corresponding to a student submission for a programming assignment can be viewed. Information regarding the category of a code save along with any results of compilation or execution can be viewed for the entire code history. Code saves may also be deleted from the system using this interface. Further, admins can grade the programming assignments using this interface. 
LEXICON DIAGRAM


Figure 16: Lexicon diagram for concepts used



==> data.tex <==
\section{Data Collection}\label{sec:data}
Describe 
\begin{enumerate}
    \item the type of data
    \item the organization of data
    \item how it can be useful
\end{enumerate}
